Data-driven Discovery of The Quadrotor Equations of Motion Via Sparse Identification of Nonlinear Dynamics

Dynamical systems provide a mathematical framework for understanding complex physical phenomena. The mathematical formulation of these systems plays a crucial role in numerous applications; however, it often proves to be quite intricate. Fortunately, data can be readily available through sensor measurements or numerical simulations. In this study, we employ the Sparse Identification of Nonlinear Dynamics (SINDy) algorithm to extract a mathematical model solely from data. The influence of the hyperparameter $\lambda$ on the sparsity of the identified dynamics is discussed. Additionally, we investigate the impact of data size and the time step between snapshots on the discovered model. To serve as a data source, a ground truth mathematical model was derived from the first principals, we focus on modeling the dynamics of a generic 6 Degrees of Freedom (DOF) quadrotor. For the scope of this initial manuscript and for simplicity and algorithm validation purposes, we specifically consider a sub-case of the 6 DOF system for simulation, restricting the quadrotor's motion to a 2-dimensional plane (i.e. 3 DOF). To evaluate the efficacy of the SINDy algorithm, we simulate three cases employing a Proportional-Derivative (PD) controller for the 3 DOF case including different trajectories. The performance of SINDy model is assessed through the evaluation of absolute error metrics and root mean squared error (RMSE). Interestingly, the predicted states exhibit at most a RMSE of order of magnitude approximately $10^{-4}$, manifestation of the algorithm's effectiveness. This research highlights the application of the SINDy algorithm in extracting the quadrotor mathematical models from data.

==> sections/Introduction.tex <==
Dynamical systems provide a mathematical representation for describing the world. Formally, dynamical systems are concerned with the analysis, and interpretation of the behavior of sets of differential equations that trace the advancement of a system's state across time \cite{arrowsmith_introduction_1990, brunton_data-driven_2019}. Classical dynamics has been discussed for years and applied to a wide range of applications; it is far too complex to be stated in a few words. However, the combination of big data, machine learning techniques, and statistical learning is driving a revolution in data-driven dynamical modeling and control of complex systems, with analytical derivations being replaced by data-driven methodology \cite{kaiser2018sparse}. In most real-world circumstances, data is so abundant that it cannot be comprehended. Furthermore, the physical principles that control these data are frequently complex; this is true for most physical concerns, such as climate science, epidemiology, and finance, to name a few. Researchers \cite{rowley2004model, rowley2017model, hayhoe2020data} attempt to decompose data in order to acquire insights into these massive, yet unexplained, datasets. As a result, the abundance of data remains a challenge because it is inherently imperfect. Consequently, the rise of data-driven dynamics is paving the way for such difficulties. 


The outcome of this development in data science was not initially noticeable on dynamical systems \cite{brunton_discovering_2016}, but recently a lot of research has been geared towards that area. Bongard and Lipson \cite{bongard2007automated} and Schmidt and Lipson \cite{schmidt2009distilling} was able to glean information about a nonlinear dynamical system's structure which was used after that to find the nonlinear differential equations \cite{koza1994genetic} by symbolic regression. Dynamic Mode Decomposition (DMD) was first introduced to fluid dynamics by Schmid \cite{schmid2008dynamic}. He extracted spatiotemporal structures from high dimensional data using DMD to analyse it. Researchers have extended the DMD method to explore other interesting intersections, including but not limited to the Koopman operator \cite{koopman_hamiltonian_1931}, extended DMD \cite{williams_datadriven_2015} to allow for approximation for Koopman operator, kernel DMD \cite{williams_kernel-based_2015, baddoo2022kernel}, time-delay DMD \cite{brunton_chaos_2017, arbabi_ergodic_2017}. Moreover, Proctor et al. \cite{proctor_dynamic_2016} extended the DMD to account for control input. These methods allow for linear system identification. Although these techniques rely on a precise set of coordinates for dynamics linearization, they are beneficial for developing dynamics-based linear models that progress high-dimensional observations across time  \cite{tu_dynamic_2014, tu2013dynamic} which are useful for control purposes \cite{champion2019data}. Recent studies \cite{yeung_learning_2017, takeishi_learning_2018} have examined the use of deep learning techniques to choose the proper set of coordinates to be used in both DMD and extended DMD.

While linear dynamical systems have several great qualities, there are many complex and intriguing dynamical phenomena that a linear model cannot properly capture. This encourages ways for discovering models of nonlinear dynamical systems. Consequently, another breakthrough on data-driven dynamics happened after Brunton et al. \cite{brunton_discovering_2016} revealed the method of discovering nonlinear equations of motion using SINDy algorithm. They combined compressed sensing \cite{candes_robust_2006, candes_stable_2006, donoho_compressed_2006} with sparse regression \cite{tibshirani_regression_1996, james_introduction_2021} and came up with the new technique of SINDy, which is based on the idea that most dynamical systems contain a small number of active terms that account for the majority of dynamics. Recently, SINDy algorithm has been generalized to include control inputs \cite{kaiser2018sparse}, to include tensor bases \cite{gelss2019multidimensional}, to discover partial differential equation \cite{rudy2017data, schaeffer2017learning}, and to account for noisy data as a kind of challenge \cite{schaeffer_sparse_2017, reinbold2020using}. The usage of SINDy algorithm thereafter begin to be a workhorse in the fields of optics, chemical engineering, robotics, and disease modeling \cite{jiang_modeling_2021, thiele_system_2020, bhadriraju_operable_2020, bhattacharya_sparse_2020, sorokina_sparse_2016}.

Despite the increasing body of literature in the field, there has been a dearth of research focused on the domain of aerospace, especially the Unmanned Aerial Vehicles (UAV). A few studies discussed data-driven dynamics and control as an application of the UAVs.

Manzoor et al. \cite{manzoor2022model} proposed a novel approach for controlling ducted fan aerial vehicles (DFAVs) by integrating model predictive control (MPC) and physics-informed machine learning. They combined the physics-based model with the data-driven model to account for sudden changes in the system dynamics motivated by \cite{quade2018sparse, kaheman2019learning}. Also, Kaiser et al. \cite{kaiser2018sparse} proposed an integration between SINDy and MPC. They found that the SINDy method needs less data compared to other popular machine learning approaches, such as neural networks. This reduces the likelihood of over-fitting. In contrast to \cite{manzoor2022model}, when combined with MPC, the SINDy algorithm yields models that are both computationally feasible and precise, even when trained on limited data. 

Motivated by this, SINDy algorithm will be utilized to discover the EOM of quadrotor using numerical simulation data at first, and for the next phase, experimental data might be used. Moreover, a study on SINDy's sparsity hyperparameter effect on model discovery will be examined along with the effect of the sampling time of data collected whether numerically or experimentally. 

%The dynamics of UAV is already known. But, there are multiple challenges for revealing the underlying uncertainties/disturbances such as the assumption of rigid body analysis and extreme non-linearities. Moreover, the basic principle of multi-copter UAV is based on the aerodynamic force generated by the rotation of multi-rotors; thus, the vehicle is extremely sensitive to the aerodynamic disturbances \cite{thanh_quadcopter_2022}. This study hypothesize that SINDy model might result on more comprehensive model compared to the simple analytical one.
